A Customizable Dynamic Scenario Modeling and Data Generation Platform for Autonomous Driving

Safely interacting with humans is a significant challenge for autonomous driving. The performance of this interaction depends on machine learning-based modules of an autopilot, such as perception, behavior prediction, and planning. These modules require training datasets with high-quality labels and a diverse range of realistic dynamic behaviors. Consequently, training such modules to handle rare scenarios is difficult because they are, by definition, rarely represented in real-world datasets. Hence, there is a practical need to augment datasets with synthetic data covering these rare scenarios. In this paper, we present a platform to model dynamic and interactive scenarios, generate the scenarios in simulation with different modalities of labeled sensor data, and collect this information for data augmentation. To our knowledge, this is the first integrated platform for these tasks specialized to the autonomous driving domain.

==> api.tex <==


Along with the dataset, a Python API is provided to facilitate quick browsing of simulation data. The API includes functions to visualize lidar point clouds, process semantic tags, and overlay bounding boxes on frame data.

==> future.tex <==
Synthesis of Scenic programs from data
==> open up possibilities of leveraging domain adaptation to enhance the practical use of simulated data for modules in downstream of autonomous stack such as behavior prediction and planner.


==> labels.tex <==
For the synthetic dataset, an RGB camera was used to record front-facing videos for the ego vehicle, along with ground-truth depth, semantic segmentation, and 2D bounding box data. In addition, a lidar sensor recorded 360-degree sweeps of the scene, including semantic labels for each point in the cloud and 3D bounding boxes. Figure \ref{fig:annotations} illustrates the provided annotations on a single frame.

\subsection{Sensor Configuration}

The video camera and lidar sensor were placed at the same location on the ego vehicle's hood, exactly 2.4 meters off the ground.

The video camera recorded 15 frames per second at a resolution of 1280x720, with a 90 degree horizontal field of view (FoV). Per-pixel-depth information and semantic labels were also captured.

The lidar sensor ran at a frequency of approximately 15 sweeps per second, recording about 22,000 points per sweep. The lower (vertical) FoV was set to -25 degrees, and the upper FoV was set to 15 degrees. Its range was set to 40 meters.

\subsection{Sensor Data Processing}

The simulator directly provided 3D bounding boxes for objects in the scene. Their coordinates are given with reference to the lidar-sensor coordinate system. Unfortunately, the simulator does not provide ground-truth 2D bounding box data. To circumvent this issue, the 3D boxes were projected onto the video camera image plane using a calibration matrix. Naturally, the 2D bounding boxes are not perfectly snug around their corresponding objects, but are likely to be sufficient for many image detection tasks.

\begin{figure}
\centering
\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{figures/frame_semantic.jpg}
\caption{Semantic Segmentation}
\label{fig:semantic}
\end{subfigure}
\begin{subfigure}[b]{.49\linewidth}
\includegraphics[width=\linewidth]{figures/frame_lidar.jpg}
\caption{Lidar with Semantic Labels}
\label{fig:lidar}
\end{subfigure}

\begin{subfigure}[b]{.32\linewidth}
\includegraphics[width=\linewidth]{figures/frame_2d_bbox.jpg}
\caption{2D Bounding Boxes}
\label{fig:bbox2d}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
\includegraphics[width=\linewidth]{figures/frame_depth.jpg}
\caption{Depth Image}
\label{fig:depth}
\end{subfigure}
\begin{subfigure}[b]{.32\linewidth}
\includegraphics[width=\linewidth]{figures/frame_3d_bbox.jpg}
\caption{3D Bounding Boxes (Projected)}
\label{fig:bbox3d}
\end{subfigure}

\caption{Collected Sensor Data and Labels using the \scenic{} program described in Figure~\ref{fig:badlyparked}}
\label{fig:annotations}
\end{figure}
